A Unified Framework for Rank-based Evaluation Metrics for Link Prediction in Knowledge Graphs

The link prediction task on knowledge graphs without explicit negative triples in the training data motivates the usage of rank-based metrics. Here, we review existing rank-based metrics and propose desiderata for improved metrics to address lack of interpretability and comparability of existing metrics to datasets of different sizes and properties. We introduce a simple theoretical framework for rank-based metrics upon which we investigate two avenues for improvements to existing metrics via alternative aggregation functions and concepts from probability theory. We finally propose several new rank-based metrics that are more easily interpreted and compared accompanied by a demonstration of their usage in a benchmarking of knowledge graph embedding models.

==> Ranking Metrics @ GLB 2022/text/acronyms.tex <==
\DeclareAcronym{MR}{
    short = MR,
    long  = mean rank
}
\DeclareAcronym{ZMR}{
    short = ZMR,
    long  = z-mean rank
}
\DeclareAcronym{MRR}{
    short = MRR,
    long  = mean reciprocal rank
}
\DeclareAcronym{ZMRR}{
    short = ZMRR,
    long  = z-mean reciprocal rank
}
\DeclareAcronym{HK}{
    short = H\textsubscript{$k$},
    long  = hits at $k$
}
\DeclareAcronym{ZHK}{
    short = ZH\textsubscript{$k$},
    long  = z-hits at $k$
}
\DeclareAcronym{AHK}{
    short = AH\textsubscript{$k$},
    long  = adjusted hits at $k$
}
\DeclareAcronym{AMRR}{
    short = AMRR,
    long  = adjusted mean reciprocal rank
}
\DeclareAcronym{AMR}{
    short = AMR,
    long  = adjusted mean rank
}
\DeclareAcronym{AMRI}{
    short = AMRI,
    long  = adjusted mean rank index
}
\DeclareAcronym{HMR}{
    short = HMR,
    long  = harmonic mean rank
}
\DeclareAcronym{GMR}{
    short = GMR,
    long  = geometric mean rank
}
\DeclareAcronym{IGMR}{
    short = IGMR,
    long  = inverse geometric mean rank
}
\DeclareAcronym{IMR}{
    short = IMR,
    long  = inverse mean rank
}
\DeclareAcronym{KGEM}{
    short = KGEM,
    long  = knowledge graph embedding model
}
\DeclareAcronym{KG}{
    short = KG,
    long  = knowledge graph
}
\DeclareAcronym{CWA}{
    short = CWA,
    long  = closed-world assumption
}
\DeclareAcronym{OWA}{
    short = OWA,
    long  = open-world assumption
}

